Parendi: Thousand-Way Parallel RTL Simulation

Hardware development critically depends on cycle-accurate RTL simulation. However, as chip complexity increases, conventional single-threaded simulation becomes impractical due to stagnant single-core performance. Parendi is an RTL simulator that addresses this challenge by exploiting the abundant fine-grained parallelism inherent in RTL simulation and efficiently mapping it onto the massively parallel Graphcore IPU (Intelligence Processing Unit) architecture. Parendi scales up to 5888 cores on 4 Graphcore IPU sockets. It allows us to run large RTL designs up to 4$\times$ faster than the most powerful state-of-the-art x64 multicore systems. To achieve this performance, we developed new partitioning and compilation techniques and carefully quantified the synchronization, communication, and computation costs of parallel RTL simulation: The paper comprehensively analyzes these factors and details the strategies that Parendi uses to optimize them.

==> sections/discussion.tex <==
\section{Discussion, Future Work, and Conclusion}\label{sec:discussion}




Our work is motivated by the growing need for a highly parallel RTL simulator to compensate for the stagnated growth of single-thread performance (\figRef{sim_rate_projection}).

We studied
We quantitatively studied simulation perform across three axes and describe how the underlying architecture could limit or enable parallel simulation.
On x64 we found that synchronization and communication can severely limit performance to less than a few tens of cores.

\begin{itemize}
    \item Tooling is not there: insane compile times
    \item Partitioning matters: and system- and architecture-level concerns need to be incorporated into partitioning even on x64
    \item Synthesis vs. Compilation: are they the same at scale?
\end{itemize}
